Unpaired Weyl fermion on an axion string in a finite lattice

Domain wall fermions use a $2n$-dimensional spacetime defect embedded in $(2n+1)$-dimensional spacetime to realize massless lattice Dirac fermions. Recent work has extended this idea to realize a single unpaired Weyl fermion in a finite lattice. Here, we realize the same using a $2n$-dimensional string defect embedded in $(2n+2)$-dimensional spacetime on a finite lattice for $n=1$. This string is a lattice version of the continuum axion string described in Callan-Harvey. Our results are obtained in a Hamiltonian formulation in Minkowski spacetime. Extending the results to Euclidean spacetime and to $n>1$ is straightforward. This work has applications to lattice chiral gauge theories and axion cosmology.

==> preamble.tex <==

\usepackage[T1]{fontenc}
%\usepackage{gfsartemisia-euler}
% WG: The above font package did not properly display the extensible bra/ket notation introduced by the braket package.
\usepackage{enumitem}
\usepackage{pifont}
\usepackage{amsmath,yhmath,braket}
\newcommand{\xmark}{\ding{55}}%

\usepackage[mathscr]{euscript}

%%%%%%%%%%%%
\makeatletter
\newcommand{\subalign}[1]{%
  \vcenter{%
    \Let@ \restore@math@cr \default@tag
    \baselineskip\fontdimen10 \scriptfont\tw@
    \advance\baselineskip\fontdimen12 \scriptfont\tw@
    \lineskip\thr@@\fontdimen8 \scriptfont\thr@@
    \lineskiplimit\lineskip
    \ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\hfil\crcr
      #1\crcr
    }%
  }%
}
\makeatother
%%%%%%%%%%%%%%

\usepackage{mathtools}
\usepackage{lmodern}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{amsfonts}
\usepackage{tocvsec2}
\usepackage{slashed}
\usepackage{cancel}
\usepackage{comment}

\newcommand{\chck}{\pmb{\checkmark}}
%\newcommand\hm{H}
\newcommand{\ZF}{(\mathbb{Z}_2)_{\rm F}}
\newcommand{\ZC}{(\mathbb{Z}_2)_{\rm C}}
\newcommand{\todo}[1]{({\bf TODO:} #1)}
\newcommand\beq{\begin{eqnarray}}
\newcommand\eeq{\end{eqnarray}} 
\newcommand{\wtg}{{\widetilde \gamma}}
\newcommand{\wts}{{\widetilde \sigma}}
\newcommand{\wtc}{{\widetilde \CC}}
\newcommand{\PP}{ {\hat P_2}}
\newcommand\qslash {\slashed{q}}
\newcommand\pslash {\slashed{p}}
\newcommand\dslash {\slashed{\partial}}
\newcommand\Dslash {\slashed{D}}
\newcommand\dsl {\slashed{\partial}}
\newcommand\Dsl {\slashed{D}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\be}{\beq}
\newcommand{\ee}{\eeq}
\newcommand\eqn[1]{\label{eq:#1}} 
\newcommand\eq[1]{eq.~(\ref{eq:#1})} 
\newcommand\Eq[1]{Eq.~(\ref{eq:#1})} 
\newcommand{\bfA}{{\mathbf A}}
\newcommand{\bfB}{{\mathbf B}}
\newcommand{\bfE}{{\mathbf E}}
\newcommand{\bfQ}{{\mathbf Q}}
\newcommand{\bfx}{{\mathbf x}}
\newcommand{\bfy}{{\mathbf y}}
\newcommand{\bfr}{{\mathbf r}}
\newcommand{\bfk}{{\mathbf k}}
\newcommand{\bfm}{{\mathbf m}}
\newcommand{\bfn}{{\mathbf n}}
\newcommand{\bfp}{{\mathbf p}}
\newcommand{\bfq}{{\mathbf q}}
\newcommand{\eV}{{\rm ~eV }}
\newcommand{\keV}{{\rm ~keV }}
\newcommand{\GeV}{{\rm ~GeV }}
\newcommand{\TeV}{{\rm ~TeV }}
\newcommand{\MeV}{{\rm ~MeV }}
\newcommand{\CA}{{\cal A}}
\newcommand{\CB}{{\cal B}}
\newcommand{\CC}{{\cal C}}
\newcommand{\CD}{{\cal D}}
\newcommand{\CE}{{\cal E}}
\newcommand{\CF}{{\cal F}}
\newcommand{\CH}{{\cal H}}
\newcommand{\CI}{{\cal I}}
\newcommand{\CJ}{{\cal J}}
\newcommand{\CK}{{\cal K}}
\newcommand{\CO}{{\cal O}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CN}{{\cal N}}
\newcommand{\CP}{{\cal P}}
\newcommand{\CG}{{\cal G}}
\newcommand{\CQ}{{\cal Q}}
\newcommand{\CR}{{\cal R}}
\newcommand{\CS}{{\cal S}}
\newcommand{\CT}{{\cal T}}
\newcommand{\CU}{{\cal U}}
\newcommand{\CV}{{\cal V}}
\newcommand{\CW}{{\cal W}}
\newcommand{\CX}{{\calX}}
\newcommand{\CY}{{\cal Y}}
\newcommand{\CZ}{{\cal Z}}
\newcommand{\CL}{{\cal L}}
\newcommand\rf[1]{{\bf [REF #1]}}
\newcommand{\tr}{{\rm tr\,}}
\newcommand{\Tr}{{\rm Tr\,}}
\newcommand{\rd}{{\rm d}}
\newcommand\vev[1]{\langle #1 \rangle}
\newcommand\bigbra[1]{\big\langle #1 \big|}
\newcommand\ebra[1]{\left \langle #1 \right|}
\newcommand\bigket[1]{\big| #1 \big \rangle}
\newcommand\eket[1]{\left| #1 \right\rangle}
\newcommand\ebraket[2]{\left \langle #1 \middle| #2 \right \rangle}
\newcommand\expect[3]{\langle #1|#2|#3\rangle}
\newcommand{\mybar}[1]{\kern 0.6pt\overline{\kern -0.6pt#1\kern -0.6pt}\kern 0.6pt}

\def\tr{\text{tr}\,}
\def\Tr{\text{Tr}\,}
\def\Re{\mathrm{Re}\,}
\def\half{\tfrac{1}{2}}
\def\LambdaQCD{\Lambda_{\rm QCD}}
\def\Seff{S_{\rm eff}}
\def\UG{U(1)_{\rm G}}
\def\U\Omega{U(1)_{\Omega}}
\def\UY{U(1)_{Y}}
\def\SI{S_{\rm I}}
\def\Vmaj{V_{\rm maj}}
\def\Vov{V_{\rm ov}}
\def\muBs{\mu_B^{\rm sat}}

\hypersetup{
  colorlinks=true,   % false: boxed links; true: colored links
  linkcolor=cyan,    % color of internal links (box color = linkbordercolor)
  citecolor=blue,    % color of links to bibliography
  filecolor=magenta, % color of file links
  urlcolor=blue      % color of external links
}
\usepackage[section]{placeins}
\newcommand{\ig}{\includegraphics}


